QCD domain walls, Chern-Simons theories and holography

Massive QCD at $\theta=\pi$ breaks CP spontaneously and admits domain walls whose dynamics and phases depend on the number of flavors and their masses. We discuss these issues within the Witten-Sakai-Sugimoto model of holographic QCD. Besides showing that this model reproduces all QCD expectations, we address two interesting claims in the literature. The first is about the possibility that the QCD domain-wall theory is fully captured by three-dimensional physics, only. The second regards the existence of quantum phases in certain Chern-Simons theories coupled to fundamental matter. Both claims are supported by the string theory construction.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%              LaTeX macros -- Ioannis Papadimitriou v. 30.05.2015
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Shortcuts

\def \bib{\bibitem}
\def\){\right)}
\def\({\left( }
\def\]{\right] }
\def\[{\left[ }
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\def\NO{\nonumber}
\def\nonu{\nonumber \\}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}

%\def\bal{\begin{align}}
%\def\eal{\end{align}}

\def\bal#1\eal{\begin{align}#1\end{align}}

\def\bald{\begin{aligned}}
\def\eald{\end{aligned}}

%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}

%\def\beqa{\begin{eqnarray}}
%\def\eeqa{\end{eqnarray}}

\def\beqx{\begin{displaymath}}
\def\eeqx{\end{displaymath}}

\newcommand{\bmat}{\left(\begin{array}}
\newcommand{\emat}{\end{array}\right)}

%\renewcommand{\theequation}{\thesection.\arabic{equation}}

\def\half{\frac{1}{2}}


% New environments

\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{conjecture}{Conjecture}[section]

% Abbreviations for Greek letters

\def\a{\alpha}
\def\b{\beta}
\def\c{\chi}
\def\d{\delta}
\def\e{\epsilon}
\def\f{\phi}
\def\g{\gamma}
\def\h{\eta}
\def\i{\iota}
\def\j{\psi}
\def\k{\kappa}
\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\o{\omega}
    \def\om{\omega}
\def\p{\pi}
\def\q{\theta}
    \def\th{\theta}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
%\def\u{\upsilon}
\def\x{\xi}
\def\z{\zeta}
\def\D{\Delta}
\def\F{\Phi}
\def\G{\Gamma}
\def\J{\Psi}
\def\L{\Lambda}
\def\O{\Omega}
    \def\Om{\Omega}
\def\P{\Pi}
\def\Q{\Theta}
    \def\Th{\Theta}
\def\S{\Sigma}
\def\U{\Upsilon}
\def\X{\Xi}

% Varletters

\def\ve{\varepsilon}
\def\vr{\varrho}
\def\vs{\varsigma}
\def\vq{\vartheta}
    \def\vth{\vartheta}
\def\tvf{\tilde{\varphi}}
\def\vf{\varphi}
    \def\vphi{\varphi}

% Greek bb letters -- requires \usepackage[bbgreekl]{mathbbol}

\def\ba{\bbalpha}
\def\bk{\bbkappa}
\def\bg{\bbgamma}
\def\bd{\bbdelta}
%\def\be{\bbepsilon}
\def\bs{\bbsigma}

% Calligraphic letters

\def\ca{{\cal A}}
\def\cb{{\cal B}}
\def\cc{{\cal C}}
\def\cd{{\cal D}}
\def\ce{{\cal E}}
\def\cf{{\cal F}}
\def\cg{{\cal G}}
\def\ch{{\cal H}}
\def\ci{{\cal I}}
\def\cj{{\cal J}}
\def\ck{{\cal K}}
\def\cl{{\cal L}}
\def\cm{{\cal M}}
\def\cn{{\cal N}}
\def\co{{\cal O}}
\def\cp{{\cal P}}
\def\cq{{\cal Q}}
\def\car{{\cal R}}
\def\cs{{\cal S}}
\def\ct{{\cal T}}
\def\cu{{\cal U}}
\def\cv{{\cal V}}
\def\cw{{\cal W}}
\def\cx{{\cal X}}
\def\cy{{\cal Y}}
\def\cz{{\cal Z}}

% Accents and foreign (in text):

% Fonts

\def\Sc#1{{\hbox{\sc #1}}}      % script for single characters in equations
\def\Sf#1{{\hbox{\sf #1}}}      % sans serif for single characters in equations
\def\mb#1{\mbox{\boldmath $#1$}}% bold math character
\def\mf#1{\ensuremath{\mathfrak{#1}}} %mathfrak
\def\bb#1{\ensuremath{\mathbb{#1}}} %mathbb

% Math symbols

\def\slpa{\slash{\pa}}                         % slashed partial derivative
\def\slin{\SLLash{\in}}                                 % slashed in-sign
\def\bo{{\raise-.3ex\hbox{\large$\Box$}}}               % D'Alembertian
\def\cbo{\Sc [}                                         % curly "
\def\pa{\partial}                                       % curly d
\def\de{\nabla}                                         % del
\def\dell{\nabla}                                       % hi ho the dairy-o
\def\su{\sum}                                           % summation
\def\pr{\prod}                                          % product
\def\iff{\leftrightarrow}                               % <-->
\def\conj{{\hbox{\large *}}}                            % complex conjugate
\def\ltap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$<$}}   % < or ~
\def\gtap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$>$}}   % > or ~
\def\face{{\raise.2ex\hbox{$\displaystyle \bigodot$}\mskip-2.2mu \llap {$\ddot
        \smile$}}}                                   % happy face
\def\dg{\dagger}                                     % hermitian conjugate
\def\ddg{\ddagger}                                   % double dagger
\def\trans{\mbox{\scri T}}                           % T for transposition
\def\>{\rangle}                                      %right angle
\def\<{\langle}                                      %left angle

% Math stuff with one argument

\def\sp#1{{}^{#1}}                                   % superscript (unaligned)
\def\sb#1{{}_{#1}}                                   % sub"
\newcommand{\sub}[1]{\phantom{}_{(#1)}\phantom{}}    % subscript in ( )
\def\oldsl#1{\rlap/#1}                               % poor slash
\def\slash#1{\rlap{\hbox{$\mskip 1 mu /$}}#1}        % good slash for lower case
\def\Slash#1{\rlap{\hbox{$\mskip 3 mu /$}}#1}        % " upper
\def\SLash#1{\rlap{\hbox{$\mskip 4.5 mu /$}}#1}      % " fat stuff (e.g., M)
\def\SLLash#1{\rlap{\hbox{$\mskip 6 mu /$}}#1}       % slash for no-in sign
\def\wt#1{\widetilde{#1}}                            % big tilde
\def\Hat#1{\widehat{#1}}                             % big hat
\def\lbar#1{\ensuremath{\overline{#1}}}              % big bar
%\def\bra#1{\left\langle #1\right|}                   % < |
%\def\ket#1{\left| #1\right\rangle}                   % | >
\def\VEV#1{\left\langle #1\right\rangle}             % < >
\def\abs#1{\left| #1\right|}                         % | |
\def\leftrightarrowfill{$\mathsurround=0pt \mathord\leftarrow \mkern-6mu
        \cleaders\hbox{$\mkern-2mu \mathord- \mkern-2mu$}\hfill
        \mkern-6mu \mathord\rightarrow$}        % <--> double differential
\def\dvec#1{\vbox{\ialign{##\crcr
        \leftrightarrowfill\crcr\noalign{\kern-1pt\nointerlineskip}
        $\hfil\displaystyle{#1}\hfil$\crcr}}}           % <--> accent
\def\dt#1{{\buildrel {\hbox{\LARGE .}} \over {#1}}}     % dot-over for sp/sb
\def\dtt#1{{\buildrel \bullet \over {#1}}}              % alternate "
\def\der#1{{\pa \over \pa {#1}}}                        % partial derivative
\def\fder#1{{\d \over \d {#1}}}                         % functional derivative
\def\tr{{\rm tr \,}}                                    % trace
\def\Tr{{\rm Tr \,}}                                    % Trace
\def\diag{{\rm diag \,}}                                % diagonal
\def\Re{{\rm Re\,}}                                     % Real part
\def\Im{{\rm Im\,}}                                     % Imaginary part

% Math stuff with more than one argument

\def\partder#1#2{{\partial #1\over\partial #2}}        % partial derivative of
\def\parvar#1#2{{\d #1\over \d #2}}                    % variation of
\def\secder#1#2#3{{\partial^2 #1\over\partial #2 \partial #3}}  % second "
\def\on#1#2{\mathop{\null#2}\limits^{#1}}              % arbitrary accent
\def\bvec#1{\on\leftarrow{#1}}                         % backward vector accent
\def\oover#1{\on\circ{#1}}                             % circle accent

% Physics related

\def\Deq#1{\mbox{$D$=#1}}                               % Dimension
\def\Neq#1{\mbox{$cn$=#1}}                              % SUSY
\newcommand{\ampl}[2]{{\cal M}\left( #1 \to #2 \right)} % Scattering amplitude

% Abbreviations for journals

\def\NPB#1#2#3{Nucl. Phys. B {\bf #1} (19#2) #3}
\def\PLB#1#2#3{Phys. Lett. B {\bf #1} (19#2) #3}
\def\PLBold#1#2#3{Phys. Lett. {\bf #1}B (19#2) #3}
\def\PRD#1#2#3{Phys. Rev. D {\bf #1} (19#2) #3}
\def\PRL#1#2#3{Phys. Rev. Lett. {\bf #1} (19#2) #3}
\def\PRT#1#2#3{Phys. Rep. {\bf #1} C (19#2) #3}
\def\MODA#1#2#3{Mod. Phys. Lett.  {\bf #1} (19#2) #3}

% Miscellaneous

\def\norder{\raisebox{-.13cm}{\ensuremath{\circ}}\hspace{-.174cm}\raisebox{.13cm}{\ensuremath{\circ}}}
\def\bz{\bar{z}}
\def\bw{\bar{w}}
\def\-{\hphantom{-}}
\newcommand{\dd}{\mbox{d}}
\newcommand{\scr}{\scriptscriptstyle}
\newcommand{\scri}{\scriptsize}
\def\rand#1{\marginpar{\tiny #1}}               % Randbemerkung
\newcommand{\rstar}{\rand{\bf\large *}}
\newcommand{\rup}{\rand{$\uparrow$}}
\newcommand{\rdown}{\rand{$\downarrow$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
